The 5G-AKA Authentication Protocol Privacy

We study the 5G-AKA authentication protocol described in the 5G mobile communication standards. This version of AKA tries to achieve a better privacy than the 3G and 4G versions through the use of asymmetric randomized encryption. Nonetheless, we show that except for the IMSI-catcher attack, all known attacks against 5G-AKA privacy still apply. Next, we modify the 5G-AKA protocol to prevent these attacks, while satisfying the cost and efficiency constraints of the 5G-AKA protocol. We then formally prove that our protocol is sigma-unlinkable. This is a new security notion, which allows for a fine-grained quantification of a protocol privacy. Our security proof is carried out in the Bana-Comon indistinguishability logic. We also prove mutual authentication as a secondary result.

==> terms.tex <==
\section{Protocol Description and Terms}

% \begin{figure}[p]
%   \begin{center}
%     \begin{tikzpicture}[>=latex]
%       \tikzset{lnode/.style={inner sep=0.2em,draw,circle}};
%       \node[draw,double] at (-0,2) {$\ue(\agent{A},\key,\mkey,\sqn_\ue)$};
%       \node[draw,double] at (8,2) {$\hn(\key,\mkey,\sqn_\hn)$};

%       \draw[<-] (0,1)
%       node[lnode,left=1.5em]{\footnotesize $\lue_0$}
%       -- ++(8,0)
%       node[midway,below]{$
%         \nonce_\id
%         $};

%       \draw[->] (0,0) -- ++(8,0)
%       node[lnode,right=1.5em] {\footnotesize $\lhn_0$}
%       node[midway,below]{$
%         \pair{\enc{\agent{A}}{\pk_\hn}{\enonce}}
%         {\mac{\spair
%             {\enc{\agent{A}}{\pk_\hn}{\enonce}}
%             {\nonce_\id}}
%           {\mkey}{1}}
%         $};

%       \draw[<-] (0,-2)
%       node[lnode,left=1.5em]{\footnotesize $\lue_1$}
%       -- ++(8,0)
%       node[draw,right=1.5em,below=2em,anchor=north west]
%       {$\sqn_\hn := \sqnsuc(\sqn_\hn)$}
%       node[midway,below]{$
%         \triplet{\nonce}
%         {\sqn_\hn \xor \ow{\nonce}{\key}}
%         {\mac{\pair{\nonce}{\sqn_\hn}}{\mkey}{2}}
%         $};

%       \draw[->] (0,-4)
%       node[align=left,draw,anchor=east,left=1.5em]
%       {If bad $\macsym$\\or out-of-sync}
%       -- ++(8,0)
%       node[midway,below]{$
%         \triplet{\nonce^\mstar}
%         {\sqn_\ue \xor \ow{\nonce^\mstar}{\key}}
%         {\mac{\triplet{\nonce}{\nonce^\mstar}{\sqn_\ue}}{\mkey}{3}}
%         $}
%       node[xshift=0.5em] (a) {};

%       \draw[->] (0,-6)
%       node[align=left,draw,anchor=east,left=1.5em]
%       {Otherwise\\$\sqn_\ue := \sqnsuc(\sqn_\ue)$}
%       -- ++(8,0)
%       node[midway,below]{$
%         \row{\nonce}{\rkey}
%         $}
%       node[xshift=0.5em] (b) {};

%       \draw [decorate,decoration={brace,amplitude=3.5pt}]
%       (a.west) -- (b.west)
%       node[midway,right=1em,lnode]{\footnotesize $\lhn_1$};
%     \end{tikzpicture}
%   \end{center}

%   \caption{A tentative fix of the 5G-AKA protocol}
%   \label{fig:fixed-aka}
% \end{figure}

\begin{figure}[p]
  \textbf{\underline{The $\supi$ Protocol}}
  \begin{center}
    \begin{tikzpicture}[>=latex]
      \tikzset{lnode/.style={inner sep=0.2em,draw,circle}};
      \node[draw,double] at (-0,3) {$\ue(\agent{A},\key,\mkey)$};
      \node[draw,double] at (8,3) {$\hn(\key,\mkey)$};

      \draw[<-] (0,2)
      -- ++(8,0)
      node[lnode,right=1.5em]{\footnotesize $\lhn_0$}
      node[midway,below]{$\nonce$};

      \draw[->] (0,1)
      node[align=left,draw,anchor=east,left=4em,yshift=1.8em]
      {\footnotesize $\sqn_\ue := \sqnsuc(\sqn_\ue)$}
      node[lnode,left=1.5em] {\footnotesize $\lue_0$}
      -- ++(8,0)
      node[align=left,draw,anchor=west,right=4em,yshift=-3em]
      {\footnotesize $\sqn_\hn := \sqnsuc(\sqn_\ue)$}
      node[midway,below]{$
        \pair
        {\enc{\pair{\agent{A}}{\sqn_\ue}}
          {\pk_\hn}{\enonce}}
        {\mac{\spair
            {\enc{\pair{\agent{A}}{\sqn_\ue}}
              {\pk_\hn}{\enonce}}
            {\nonce}}
          {\mkey}{1}}$};

      \draw[<-] (0,-2)
      -- ++(8,0)
      node[lnode,right=1.5em]{\footnotesize $\lhn_1$}
      node[midway,below]{$
        \mac{\pair{\nonce}{\sqn_\hn}}{\mkey}{2}$};

      \draw[->] (0,-3)
      node[lnode,left=1.5em]{\footnotesize $\lue_1$}
      % node[align=left,draw,anchor=east,left=4em,yshift=-3em]
      % {\footnotesize $\auth_\ue := \nonce$}
      -- ++(8,0)
      node[midway,below]{$\textsf{ok}$};
    \end{tikzpicture}
  \end{center}

  \vspace{1em}
  \textbf{\underline{The $\suci$ Protocol}}
  \begin{center}
    \begin{tikzpicture}[>=latex]
      \tikzset{lnode/.style={inner sep=0.2em,draw,circle}};
      \node[draw,double] at (-0,2) {$\ue(\agent{A},\key,\mkey)$};
      \node[draw,double] at (8,2) {$\hn(\key,\mkey)$};

      \draw[->] (0,1)
      node[lnode,left=1.5em]{\footnotesize $\lue_0$}
      -- ++(8,0)
      node[midway,below]{$
        \suci
        $};

      \draw[<-] (0,0)
      node[align=left,draw,anchor=east,left=4em,yshift=-3em]
      {\footnotesize if $\range{\sqn_\ue}{\sqn_\hn}$:\\
        \footnotesize $\sqn_\ue := \sqnsuc(\sqn_\ue)$}
      -- ++(8,0)
      node[lnode,right=1.5em] {\footnotesize $\lhn_0$}
      node[midway,below]{$
        \triplet
        {\nonce}
        {\sqn_\hn \oplus \ow{\nonce}{\key}}
        {\mac{\striplet
            {\nonce}{\sqn_\hn}{\suci}}
          {\mkey}{3}}
        $};

      \draw[->] (0,-2)
      node[lnode,left=1.5em]{\footnotesize $\lue_1$}
      -- ++(8,0)
      node[align=left,draw,anchor=west,right=4em,yshift=-2em]
      {\footnotesize $\sqn_\hn := \sqnsuc(\sqn_\hn)$}
      node[midway,below]{$
        \mac{\nonce}{\mkey}{4}
        $};

      \draw[<-] (0,-3.6)
      -- ++(8,0)
      node[lnode,right=1.5em]{\footnotesize $\lhn_1$}
      node[midway,below]{$
        \textsf{ok}
        $};

    \end{tikzpicture}
  \end{center}

  \vspace{1em}
  \textbf{\underline{The \refresh Protocol}}
  \begin{center}
    \begin{tikzpicture}[>=latex]
      \tikzset{lnode/.style={inner sep=0.2em,draw,circle}};
      \node[draw,double] at (-0,2) {$\ue(\agent{A},\key,\mkey)$};
      \node[draw,double] at (8,2) {$\hn(\key,\mkey)$};

      \draw[<-] (0,1)
      node[align=left,draw,anchor=east,left=4em,yshift=-3em]
      {\footnotesize $\success_\ue := \true$\\
        \footnotesize $\suci_\ue := \suci$}
      -- ++(8,0)
      node[lnode,right=1.5em]{\footnotesize $\lhn$}
      node[midway,below]{$
        \pair
        {\suci \oplus \row{\nonce}{\key}}
        {\mac{\pair{\suci}{\nonce}}{\mkey}{5}}$}
      node[align=left,draw,anchor=west,right=4em,yshift=-3em]
      {% \footnotesize $\success_\hn := \true$\\
        \footnotesize $\suci_\hn := \suci$};

      \draw[->] (0,-1.2)
      node[lnode,left=1.5em]{\footnotesize $\lue$}
      -- ++(8,0)
      node[midway,below]{$
        \textsf{ok}
        $};
    \end{tikzpicture}
  \end{center}

  \caption{\label{fig:fixed-aka}The new version of the AKA protocol}
\end{figure}



% \begin{figure}[tb]
%   \noindent
%   \underline{\textbf{Injective authentication of the network by the user:}}
%   \begin{gather*}
%     \sucauth_\tau(\ID) \;\;\equiv\;\;
%     \instate_\tau(\eauth_\ue^\ID) \ne \fail\\
%     \auth_\tau(\ID,j) \;\;\equiv\;\;
%     \instate_\tau(\bauth_\hn^j) = \ID \wedge
%     \instate_\tau(\nonce^j_\hn) = \instate_\tau(\eauth_\ue^\ID)\\
%     \injauth_\tau(\ID,j) \;\;\equiv\;\;
%     \auth_\tau(\ID,j)
%     \;\wedge\; \bigwedge_{i \ne j}
%     \neg\auth_\tau(\ID,i)
%   \end{gather*}
%   Then we have:
%   \[
%     \forall \ID \in \iddom,\;\;
%     \sucauth_\tau(\ID)
%     \;\ra\;
%     \bigvee_{j \in \mathbb{N}}
%     \injauth_\tau(\ID,j)
%   \]
%   \underline{\textbf{Authentication of the user by the network:}}
%   \[
%     \forall \ID \in \iddom,\;
%     \instate_\tau(\eauth_\hn^j) = \ID \;\ra\;
%     \bigvee_{\tau' \le_\tau \tau} \instate_{\tau'}(\bauth_\ue^\ID) = \instate_\tau(\nonce^j_\hn)
%   \]
%   \underline{\textbf{Correction of the \textsc{refresh} protocol:}}
%   \[
%     \success_\ue^\ID \; \ra \;
%     \left(
%       \success_\hn^\ID \wedge \suci_\ue^\ID = \suci_\hn^\ID
%     \right)
%   \]
%   \underline{\textbf{User unlinkability:}}
%   \[
%     \inframe_\tau,\su_\tau \sim \inframe_\tau',\su_\tau'
%     \qquad\qquad
%     \su_\tau \;\equiv\;
%     \left(
%       \ite{\instate_\tau(\success_\ue^\ID)}{\instate_\tau(\suci_\ue^\ID)}{\fail}
%     \right)_{\ID \in \iddom}
%   \]
%   \caption{Security Properties}
%   \label{fig:sec-prop}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
